White paper: Gaia and the end states of stellar evolution

This is the product of a Gaia GREAT workshop on "Gaia and the end states of stellar evolution" held at the University of Leicester in April 2011.

==> section_population.tex <==
\section{Population synthesis}



\putbib[population_refs]

